Task Me Anything

Benchmarks for large multimodal language models (MLMs) now serve to simultaneously assess the general capabilities of models instead of evaluating for a specific capability. As a result, when a developer wants to identify which models to use for their application, they are overwhelmed by the number of benchmarks and remain uncertain about which benchmark's results are most reflective of their specific use case. This paper introduces Task-Me-Anything, a benchmark generation engine which produces a benchmark tailored to a user's needs. Task-Me-Anything maintains an extendable taxonomy of visual assets and can programmatically generate a vast number of task instances. Additionally, it algorithmically addresses user queries regarding MLM performance efficiently within a computational budget. It contains 113K images, 10K videos, 2K 3D object assets, over 365 object categories, 655 attributes, and 335 relationships. It can generate 750M image/video question-answering pairs, which focus on evaluating MLM perceptual capabilities. Task-Me-Anything reveals critical insights: open-source MLMs excel in object and attribute recognition but lack spatial and temporal understanding; each model exhibits unique strengths and weaknesses; larger models generally perform better, though exceptions exist; and GPT4o demonstrates challenges in recognizing rotating/moving objects and distinguishing colors.

==> submission-sections/case-study-syn2real.tex <==
\section{A Case Study for Synthetic Data vs. Real Data in \name}
\label{sec:discuss-syn2real}
\name leverages both synthetic and real images/videos for evaluating MLM models. While synthetic data are higly controllable, low-cost, its effectiveness compared to real data remains unclear, particularly given that most benchmarks rely heavily on real datasets. In this section, we present 3 different experiments to compare synthetic and real data, demonstrating the effectiveness and reliability of synthetic data in MLM model evaluation.

\subsection{Correlation analysis: synthetic vs. real image/video}
\begin{figure}[!h]
  \centering
  \begin{minipage}{0.38\linewidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/syn2real/TaskMeAnything rebuttal figure1.png}
    \caption{Correlations of synthetic data with real data in \name.}
    \label{fig:cor-within-tma}
  \end{minipage}%
  \hfill
  \begin{minipage}{0.52\linewidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/syn2real/TaskMeAnything rebuttal figure2.png}
    \caption{Correlations of \name with other popular MLM benchmarks.}
    \label{fig:cor-with-other-benchmarks}
  \end{minipage}
\end{figure}
To quantitatively justify the transferability between evaluations on synthetic and real-world images, we compared 18 models’ rankings on synthetic vs. realistic images and obsered strong positive correlations between them. Across the three different image sources in Task-Me-Anything, we found that the correlation between models’ rankings on 2D and 3D synthetic images is the strongest (r=0.99). While the correlations between models’ rankings on real and 2D images, and between real and 3D images are slightly smaller (r=0.85 and 0.79 respectively), these numbers still suggest strong positive correlations between models’ performance on synthetic images and on real images (Figure~\ref{fig:cor-within-tma}, Figure~\ref{fig:cor-with-other-benchmarks}).

% \subsection{Counting Performance in \name Compared to TallyQA}
% Similarly, we have also conducted a comparative analysis of models’ “counting” performance on Task-Me-Anything’s synthetic images vs. on TallyQA’s realistic images, which are all human-annotated. Again, we found that models’ performance on our synthetic scenes is highly correlated with their performance on TallyQA (r=0.714). See the Appendix~\ref{app:tallyqa} for additional details on this analysis.


% \subsection{Human evaluation}
% Last but not least, in addition to strong correlations with evaluations using real images, we argue that our evaluation with synthetic images offers two unique advantages over real images. First, our human evaluation shows that human annotators achieve near-perfect performance (99.4, 99.73, 97.33\%) across all image sources, including the synthetic ones, whereas MLMs perform relatively poorly on 2D and 3D synthetic images compared to real images. This suggests that our evaluation with synthetic images consists of reasonable tasks that are especially challenging to the models. 

==> tables/query-example.tex <==
\begin{table*}[!h]
  \centering
  \small
  \caption{The query types and example queries.}
  % \scalebox{0.65}{
  \resizebox{\linewidth}{!}{
    \begin{tabular}{ll} 
    \toprule
    {\bf Query type} & {\bf Example} \\ 
    \midrule

    \multirow{1}{*}{Top-K}  
    & Return the top 10 tasks where the model $M1$ performs the worst.\\ 
    \midrule
    
    \multirow{1}{*}{Threshold} 
    & Return all the relation types where the minimum performance of models $M1$ and $M2$ is below 50\%.\\ 
    \midrule
    
    \multirow{1}{*}{Model Comparison} 
    & Return all the tasks where model $M1$ consistently outperforms $M2$ by a margin larger than 30\%.\\ 
    \midrule
    
    \multirow{1}{*}{Model Debugging} 
    & Return all the tasks where model $M1$'s performance is more than one standard deviation below its average performance.\\ 
    \midrule
    

\end{tabular}
}
  \label{tab:query-example}
\end{table*}
